One for All: Simultaneous Metric and Preference Learning over Multiple Users

This paper investigates simultaneous preference and metric learning from a crowd of respondents. A set of items represented by $d$-dimensional feature vectors and paired comparisons of the form ``item $i$ is preferable to item $j$'' made by each user is given. Our model jointly learns a distance metric that characterizes the crowd's general measure of item similarities along with a latent ideal point for each user reflecting their individual preferences. This model has the flexibility to capture individual preferences, while enjoying a metric learning sample cost that is amortized over the crowd. We first study this problem in a noiseless, continuous response setting (i.e., responses equal to differences of item distances) to understand the fundamental limits of learning. Next, we establish prediction error guarantees for noisy, binary measurements such as may be collected from human respondents, and show how the sample complexity improves when the underlying metric is low-rank. Finally, we establish recovery guarantees under assumptions on the response distribution. We demonstrate the performance of our model on both simulated data and on a dataset of color preference judgements across a large number of users.

==> sections/conclusion.tex <==
\section{Discussion}
\label{sec:conclusion}

\todo{Major discussion point: item count amelioration. How can we reduce $\Omega(d^2)$ item requirement?} \\
\todo{@Greg low-rank sensing, we expect only $dr$ items, intuition from selection matrices requiring $dr + r + 1$ for $dr + r$ DOF and possibly reference experimental evidence (may be in appendix)} \\
\todo{@Blake remark on triplets: triplets only need $\Omega(r)$ items in low-rank case (cite this result from Learning Low). Maybe we can mix and match triplets and pairs to bring overall item cost down? Future work.}

\todo{Conclusion statements}
